Reconciling Modern Deep Learning with Traditional Optimization Analyses: The Intrinsic Learning Rate

Recent works (e.g., (Li and Arora, 2020)) suggest that the use of popular normalization schemes (including Batch Normalization) in today's deep learning can move it far from a traditional optimization viewpoint, e.g., use of exponentially increasing learning rates. The current paper highlights other ways in which behavior of normalized nets departs from traditional viewpoints, and then initiates a formal framework for studying their mathematics via suitable adaptation of the conventional framework namely, modeling SGD-induced training trajectory via a suitable stochastic differential equation (SDE) with a noise term that captures gradient noise. This yields: (a) A new ' intrinsic learning rate' parameter that is the product of the normal learning rate and weight decay factor. Analysis of the SDE shows how the effective speed of learning varies and equilibrates over time under the control of intrinsic LR. (b) A challenge -- via theory and experiments -- to popular belief that good generalization requires large learning rates at the start of training. (c) New experiments, backed by mathematical intuition, suggesting the number of steps to equilibrium (in function space) scales as the inverse of the intrinsic learning rate, as opposed to the exponential time convergence bound implied by SDE analysis. We name it the Fast Equilibrium Conjecture and suggest it holds the key to why Batch Normalization is effective.

==> broader.tex <==
\section*{Broader Impact}

The observation of this paper may help understanding the generalization of deep learning and make hyper-parameter tuning easier for both researchers and practitioners.

==> chaotic.tex <==
\section{Full Batch Gradient Descent $\neq$ Gradient Flow} \label{sec:full-batch}

It's well known that for $L$-smooth objectives, one can pick an enough small LR ($\eta\le \frac{1}{L}$) such that the trajectory of gradient descent will be close to that of gradient flow. But for normalized networks, the loss function is scale-invariant, thus provably non-smooth around origin (i.e. infinitely large smoothness) \citep{li19learningrate}. Though \citet{arora2018theoretical} showed that norm will monotone increase without WD for SGD, but \citet{li19learningrate} argued that the norm will unavoidably enter the non-smooth region with WD. In this section, we argue that this issue of WD can make the training unstable and even chaotic for  full-batch GD, no matter how small the learning rate is. Meanwhile, the convergence of gradient flow is not affected, thus giving a clear separation between the trajectories of GD and gradient flow.

\textbf{The Arise of Chaos: Unbounded Smoothness} We start with a simple 2-variable scale-invariant objective, $L(x,y) = \frac{x^2}{x^2+y^2}$, and we only care about the direction of $(x,y)$, or equivalently $\frac{x}{y}$. It's clear for Gradient Flow $|\frac{x_t}{y_t}|$ monotone decreases even with WD turned on. But for GD with WD, one can see from \Cref{subfig:chaotic_toy} that once the trajectory gets close to origin, the original tiny difference is amplified and the trajectories start to diverge, meaning the dynamics of GD with WD is super-sensitive to the initialization.

We verify the same behavior on modern deep nets too, see \Cref{subfig:chaotic_gd_acc,subfig:chaotic_gd_norm}. The training dynamics oscillates between full accuracy and low accuracy, because whenever the accuracy is full for a long period, the norm becomes very small due to small gradients, and thus the effective LR gets larger  and the loss increases.
\begin{figure}
        \centering
        \begin{subfigure}[b]{0.27\textwidth}
                \centering
				\includegraphics[width=\linewidth]{tmp_images/chaotic_toy.png}
				\caption{GD with WD on $L(x,y)$ for 100 steps}
				\label{subfig:chaotic_toy}
        \end{subfigure}%
        \begin{subfigure}[b]{0.34\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/gd_chaotic_acc.png}
                \caption{Train accuracy}
                \label{subfig:chaotic_gd_acc}
        \end{subfigure}%
        \begin{subfigure}[b]{0.34\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/gd_chaotic_norm.png}
                \caption{Norm}
                \label{subfig:chaotic_gd_norm}
        \end{subfigure}%
        \caption{ WD makes SGD on scale invariant loss unstable and chaotic, for both the toy model and PreResNet32. (a).  Toy model is trained GD with $0.1$ LR and $0.5$ WD. Note that both initialization are very close to each other and the the global minimum of $L$. (b),(c). \emph{Convergence never truly happens} for PreResNet32 trained on sub-sampled CIFAR10 containing 1000 images with full-batch GD with 0.0005 WD and 1.6 LR, without momentum. PreResNet32 could easily gets to $100\%$ training accuracy, but just unable to stay long. WD is turned off at epoch 30000.}
        \label{fig:chaotic}
\end{figure}


\textbf{Weakness of the current framework.} Our approximation for SGD by SDE only works well when the noise dominates the gradient, because from \Cref{eq:sgd-sde} one can see that when there's no noise, the approximation is just to use Gradient Flow to approximate Gradient Descent with any LR. This mismatch also can been seen through the evolution of the norms (See in Appendix). In \Cref{subfig:chaotic_gd_norm}, we found without noise, the norm in GD still roughly keeps at some constant size. [One way to resolve this issue is to model a single step GD as stochastic process. We leave a more detailed justification for this in appendix.] \zhiyuan{Do we need this? Can delete it.}





==> old_experiments.tex <==
\section{Experiments with BN}

Suppose we have three learning rates: $\eta_1, \eta_2, \eta_3$, corresponding to large-scale, medium-scale and small-scale learning rate.

\begin{figure}
\centering
\includegraphics[width = 0.7\linewidth]{tmp_images/gap1.png}	
\caption{Canonical LR decay leads to a temporary increase in test accuracy}\label{fig:gap1}
\end{figure}


\begin{figure}
        \centering
        \begin{subfigure}[b]{0.49\textwidth}
                \centering
				\includegraphics[width=\linewidth]{tmp_images/init_small_lr}
        \end{subfigure}%
        \begin{subfigure}[b]{0.49\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/init_small_lr_norm}
        \end{subfigure}%
        \caption{To be added.}
        \label{fig:init_small_lr}
\end{figure}

\subsection{Experiment I, \Cref{fig:gap1}}

Fix the canonical weight decay $\lambda$. Compare the following:
\begin{enumerate}
	\item Use a large learning rate $\eta_1$, and then decay the learning rate to $\eta_2$.
	\item Use $\eta_2$ to train the model directly.
\end{enumerate}

The performances are the same.

\subsection{Experiment II, \Cref{fig:gap1}}

Fix the canonical weight decay $\lambda$. Initialize the model randomly. May train it using a large learning rate $\eta_1$ or not. Compare the following:
\begin{enumerate}
	\item Use the learning rate $\eta_2$ to train the model for sufficiently long time and then decay the learning rate to $\eta_3$.
	\item Use the learning rate $\eta_2$ to train the model for sufficiently long time and then decay the learning rate to $\eta_3$, meanwhile setting $\lambda = 0$. \footnote{setting $\lambda = 0$ performs equally well as early-stopping when the training accuracy goes to 100\%, throughout all experiments here.}
\end{enumerate}

1 and 2 have the same best test acc. But 1 can only achieve the best test acc in a short time interval. This suggests that we should use the second way to get a stable outcome. 


\begin{figure}
        \centering
        \begin{subfigure}[b]{0.49\textwidth}
                \centering
				\includegraphics[width=\linewidth]{tmp_images/hybrid500_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.49\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/hybrid500_2}
        \end{subfigure}%
        \caption{\hybrid\ is a hand-cradfted LR(WD) schedule for the purpose of studying whether dividing LR and WD by $\sqrt{10}$ (we call it a mixed decay) can let the norm converge to its stationary value faster, compared to the standard practice dividing the norm by 10(LR decay), or dividing the WD by 10(WD decay).}
        \label{fig:hybrid_500}
\end{figure}

The table below explains the training schedules. \footnote{The default initial hyper-parameters are lr = 0.1, wd = 0.0005, momentum =0.9}

\begin{table}[!htbp]
\centering
	\begin{tabular}{c|| c c c}
		Epoch & 0 &  80 & 300 \\
		\hline
		\hybrid & - & WD decay & mixed decay \\
		 \blue{lr\_0\_0\_lr\_0\_2000}  &  LR decay *2 & - & - \\
		\orange{wd\_80\_300\_lr\_2000} & - & WD decay & WD decay \\
		\hline
	\end{tabular}
	\caption{Schedules in \Cref{fig:hybrid_500}}
\end{table}

\begin{figure}[!htbp]
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
                \centering
				\includegraphics[width=\linewidth]{tmp_images/hybrid6000_1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.54\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/hybrid6000_2}
        \end{subfigure}%
		\caption{\red{hybrid} is the same as the \green{hybrid} in the first 500 epochs as that in \Cref{fig:hybrid_500}.}
        \label{fig:hybrid_6000}
\end{figure}

\begin{table}[!htbp]
\centering
	\begin{tabular}{c|| c c c c c}
		Epoch & 0 &  80 & 300 & 2000 & 5000\\
		\hline
		 \blue{lr\_0\_0\_5000\_8000}  &  LR decay *2 & - & -  & - & LR decay\\
		\orange{wd\_0\_lr\_0\_5000\_8000} & LR decay+ Wd decay & - & -  & -& LR decay\\
		\green{wd\_0\_0\_lr\_5000\_8000} & WD decay*2 & - & - &  - &  LR Decay\\
		\red{hybrid} & -  & WD decay & mixed decay  & mixed decay & -\\
		\hline
	\end{tabular}
	\caption{Schedules in \Cref{fig:hybrid_500}}
\end{table}
\subsection{Experiment III, No Figure}

Fix the canonical weight decay $\lambda$. Initialize the model randomly. May train it using a large learning rate $\eta_1$ or not. Compare the following:
\begin{enumerate}
	\item Use the learning rate $\eta_3$ and the canonical weight decay $\lambda = 0$ to train the model.
	\item Use the learning rate $\eta_2$ to train the model until the norm converges, and then decay the learning rate to $\eta_3$ and set $\lambda = 0$ .
	\item Use the learning rate $\eta_2$ to train the model. Far before the norm converges (to the stationary value of $\eta_2$), decay the learning rate to $\eta_3$ and set $\lambda = 0$.
\end{enumerate}

2 is the best. 3 is indeed similar to 1, and might be slightly better, because 1 can be viewed as trained with $\eta_3$ with 0 steps.  Don't have images ready for this claim. 


\subsection{Experiment IV, \Cref{fig:hybrid_500}}

\kaifeng{Is there any experiment showing that $\Tr(\Sigma_{\hW})$ is indeed a constant?}

\zhiyuan{Unfortunately, it might not be true.} The norm \green{hybrid} of hybrid decays after a mixed decay, i.e., diving LR and WD by $\sqrt{10}$ respectively. If the $\Tr(\Sigma_{\hW})$ is independent of $LR* = WD\eta\lambda$, then we expect to see the norm keeps the same value. 
\subsection{Experiment V}

Is SGD walking around some basin after sufficiently long time?

\zhiyuan{The answer is not clear.}

\begin{itemize}
	\item Positive Evidence 1: Stochastic Weight Averaging(SWA) improves test accuracy, while SWA between trajectories from different init would harm test acc.
			\begin{figure}
				\centering
				\includegraphics[width = 0.8\textwidth]{tmp_images/SWA_acc}
				\caption{SWA improves test acc. Test acc of SWA over nets from epoch 2000 to epoch $T$ plotted.  Trained with the default hyper-parameters without any LR/WD decay on CIFAR10.}
				\label{fig:swa_acc}
			\end{figure}
			
	\item Positive Evidence 2: The train/test error landscape looks almost quasi-convex (sub-level set is convex) in subspaces spanned by different nets along the same SGD trajectories. 
		
			\begin{figure}
				\centering
				\includegraphics[width = 1.2\textwidth]{tmp_images/SWA_best}
				\caption{The train/test error landscape looks convex.}
				\label{fig:swa_best}
			\end{figure}
	\item Negative Evidence 1: Even SWA works, the weights keeps moving for thousands of epochs, or millions of iterations.
				\begin{figure}
				\centering
				\includegraphics[width = 0.8\textwidth]{tmp_images/SWA_dist}
				\caption{Weights keeps moving at plateau. Heatmap of pairwise distance between networks. Trained with the default hyper-parameters without any LR/WD decay on CIFAR10. Unit in X/Y axis means 100 epochs.}
				\label{fig:swa_dist}
			\end{figure}
	\item Negative Evidence 2: For 2-layer linear net with WD but without BN, SWA harms test acc after 200000 iterations. (I renormalize the network before measuring the loss) And one can prove that SWA shouldn't hold in this case, as there's a continuous symmetry (rotational invariance) for linear net. Any stationary distribution should be rotational invariant, and it's not hard to show that there's a bump in test loss along the line segment connecting the best 2-linear net and its rotated version. 
\end{itemize}


Fix the canonical weight decay $\lambda$. Initialize the model randomly. May train it first using a large learning rate $\eta_1$ or not.

Train the model with the learning rate $\eta_2$ for a sufficiently long time. Store the model at every epoch $W_T, W_{T+1}, W_{T+2}, \dots$ after epoch $T$. Plot the relationship between the minimum, maximum, average values of $\dotp{\hW_t}{\hW_{t+k}}$ and $k$.

The inner product is increasing with $k$. So the noise drives SGD to explore even if the loss seems to converge.

\subsection{Summary}

Through experiments I - IV, we show that the best practice for training batch-normalized network is the following:
\begin{enumerate}
	\item Fix $\lambda > 0$ and use a medium-scale learning rate $\eta_2$ to train the model. Possibly use a larger effective weight decay in the beginning to speed up the training.
	\item When the norm converges, set $\lambda = 0$ and decay the learning rate to a small-scale. Train the model until convergence.
\end{enumerate}

In the first phase, SGD explores the loss landscape thanking to the noise. In the second phase, we fine-tune the model we got to get a slightly better performance.

\section{Experiments without BN}

Now we turn to ordinary networks without BN.

\subsection{Experiment I}

There is no loss plateau.

Experiment I for BN does not hold.

\subsection{Experiment II}

Is SGD walking around some basin after sufficiently long time?

\subsection{Experiment III}

Adding weight decay and additive Gaussian noise to replicate the situation of batch-normalized network.


==> sde_view.tex <==
\section{SDE-based framework for modeling SGD on Normalized Networks} \label{sec:theory}

In this section, we first focus on SGD with constant learning rate $\eta$, i.e., $\eta_t = \eta$ for all $t$ in~\eqref{eq:sgd-noisy}, and then we extend the scope of our discussion to SGD with Step Decay schedule.
%First, we review how SGD is approximated by SDE in the traditional view. 




%\kaifeng{I comment out the two remarks. I think they are unrelated to the main topic?}

\begin{comment}
We can approximate SGD by the stochastic differential equation below, where for $\vW_t\in \R^d$, $\mSigma_{\vW_t}$ is the covariance matrix of noise at $W_t$.

\begin{itemize}
    \item SGD: $\vw_{t+1} = \vw_t - \eta \left(\nabla \Loss(\vw_t) + \vxi_t\right)$, where $\vxi_t \sim N(\vzero, \mSigma_{\vw_t})$.
    
    \item SDE (Surrogate for SGD): 
    
         $\dd \vW_{t} = - \eta \left(\nabla \Loss(\vW_t) \dd t+ (\mSigma_{\vW_t})^{\frac{1}{2}} \dd \vB_t\right)$, where $\vB_t$ is the Wiener Process (Brownian motion), satisfying that $\vB_t - \vB_s \sim N(\vzero, (t-s) \mI_d)$.
\end{itemize}

\begin{remark}
	$\dd \vW'_{t} = - \nabla \Loss(\vW'_t)\dd t + \sqrt{\eta} (\mSigma_{\vW'_t})^{\frac{1}{2}} \dd B_t$ describes the same dynamics as the above equation does, except a rescaling in time, i.e.$ \vW'_{\eta t} = \vW_t$.
\end{remark}

\begin{remark}
	The above SDE is not the limit of SGD with infinite small LR. The limit of SGD is GF. To keep the stochasticity when $\eta\to 0$, we need to use SGLD,
	\[
		\vW_{t+1} = \vW_t - \eta \nabla \Loss(\vW_t) + \sqrt{\eta}\vxi_t,
	\] 
	
	whose limiting dynamics is 
	% \[ \dd W_{t} = - \eta \nabla L(\vW_t)\dd t + \sqrt{\eta}(\mSigma_{\vW_t})^{\frac{1}{2}} \dd B_t ,\]
	
	% or 
	\[ \dd \vW_{t} = - \nabla \Loss(\vW_t)\dd t +  (\mSigma_{\vW_t})^{\frac{1}{2}} \dd B_t.\]
	
	Here the noise per step increases as $\eta\to 0$. Typically one needs to manually add noise in SGLD.
\end{remark}
\end{comment}

\subsection{Re-parameterization for Weight Decay using Intrinsic Learning Rate}

For SGD with learning rate $\eta$ and weight decay $\lambda$,  we define $\lambda_e := \eta\lambda$ to be the \textit{effective weight decay}. This is actually  the original definition of weight decay~\citep{hanson1989comparing} and is also proposed (based upon experiments) in \citep{loshchilov2018decoupled} as a way to improve generalization for ADAM and SGD.
%To avoid ambiguity, we refer $\lambda$ as the \textit{canonical weight decay}.
In Section \ref{subsec:SDE_WD_Norm}, we will suggest calling $\lambda_e$ the \emph{intrinsic learning rate} because it controls
trajectory in a manner similar to learning rate.
%and suggest calling $\lambda_e$ 
%the evolution of effective learning rate (defined there), and for this reason we also call 
%For SGD with weight decay $\lambda$, 
Now we can rewrite update rule \eqref{eq:sgd-wd} and its corresponding SDE as
\begin{align} 
\vw_{t+1} &\gets (1 - \lambda_e)\vw_t - \eta \left(\nabla \Loss(\vw_t) + \vxi_t \right). \label{eq:sgd-wd-noisy} \\
\dd \vW_{t} &= - \eta \left(\nabla \Loss(\vW_t) \dd t+ (\mSigma_{\vW_t})^{\frac{1}{2}} \dd \vB_t\right) - \lambda_e \vW_t. \label{eq:sde-wd}
\end{align}

\subsection{SDE with Weight Decay and Normalization}\label{subsec:SDE_WD_Norm}

When the loss function is scale-invariant, % due to the use of normalization schemes,
the gradient noise $\mSigma_{\vW}$ is inherently anisotropic and position-dependent: Lemma~\ref{lem:perp_cov} in the appendix shows the noise lies in the subspace perpendicular to $w$ and blows up close to the origin. To get an SDE description closer to the canonical format, we reparametrize parameters to unit norm.  Define $\hW_t = \frac{\vW_t}{\norm{\vW_t}}$, $G_t = \norm{\vW_t}^2$, where $\norm{\vw}$ stands for the $\normltwo$-norm of a vector $\vw$. The following Lemma is proved in the Appendix; the proof uses It\^{o}'s Lemma and involves decoupling the dynamics into radial %(i.e., towards origin) 
and tangential components. 

\begin{lemma} The evolution of the system can be described as:
\begin{align}
\dd \hW_{t} &= - \frac{\eta}{G_t} \left(\nabla \Loss(\hW_t)\dd t + (\mSigma_{\hW_t})^{\frac{1}{2}} \dd B_t\right) - \frac{\eta^2}{2G_t^2}  \Tr(\mSigma_{\hW_t}) \hW_t\dd t \label{eq:sde-hW} \\
\frac{\dd G_t}{\dd t} &= -2 \lambda_e G_t + \frac{\eta^2}{G_t}\Tr(\mSigma_{\hW_t}) \label{eq:sde-rho}
\end{align}
where $\Tr(\mSigma_{\vw})$ is the trace of the covariance matrix at $\vw$.
(Note: $\Tr(\mSigma_{\vw}) = \E\left[\norm{\nabla \Loss(\vw; \Batch) - \nabla \Loss(\vw)}^2\right]$, so it is also a noise term.)
\end{lemma}

The SDE enables clean mathematical demonstration of many properties of normalization schemes. 
For example, dividing both sides of \eqref{eq:sde-rho} by $\eta$ gives
\begin{equation}
\frac{\dd(G_t/\eta)}{\dd t} = -2 \lambda_e \cdot \frac{G_t}{\eta} + \frac{\eta}{G_t}\Tr(\Sigma_{\hW_t}).
\end{equation}
This shows that the dynamics only depends on the ratio $G_t/\eta$, which also suggests that {\em initial LR is of limited importance, indistinguishable from scale of initialization.}  Now define $\gamma_t := (G_t/\eta)^2$. (Note that $G_t/\eta = \gamma_t^{-0.5}$ was called the \emph{effective learning rate} in \citep{hoffer2018norm,zhang2018three,arora2018theoretical}.) This simplifies the equations:
%We can further simplify the equation by replacing $(G_t/\eta)^2$ by $\gamma_t$, and we call $\gamma_t^{-0.5}$ the \emph{effective learning rate}, as in \citep{hoffer2018norm,zhang2018three,arora2018theoretical}:
\begin{align}
\dd \hW_{t} &= - \gamma_t^{-1/2} \left(\nabla L(\hW_t)\dd t + (\Sigma_{\hW_t})^{\frac{1}{2}} \dd B_t\right) - \frac{1}{2\gamma_t}  \Tr(\Sigma_{\hW_t}) \hW_t\dd t. \label{eq:gamma_W} \\
\frac{\dd \gamma_t}{\dd t} &= -4 \lambda_e \gamma_t + 2 \Tr(\Sigma_{\hW_t}) \label{eq:gamma}.
\end{align}
Arriving at such a point many analyses of SDEs in deep learning (for example ~\citep{chaudhari2018stochastic}) will make the simplifying assumption that the noise matrix  $\Sigma_{\hW_t}$ is the same for all $hW_t\in \sphS^{d-1}$, often even that it is identity $I$ ({\em isotropic noise}). Our experiments show that such assumptions are far from true. However, a much weaker assumption turns out to suffice, namely about the {\em trace} of the noise matrix.

\eqref{eq:gamma} can be alternatively written as the following, which shows that squared effective LR is a running average of the norm squared of gradient noise.
%This resembles RMSprop~\citep{hinton2012rmsprop} and Adam~\citep{kingma2014adam} in which a similar quantity is used for coordinatewise adaptive LR.
\begin{equation} \label{eq:gamma-avg}
	\gamma_t = e^{-4 \lambda_et} \gamma_0 + 2 \int_{0}^{t} e^{-4 \lambda_e (t-\tau)} \Tr(\Sigma_{\hW_{\tau}}) d\tau.
\end{equation}

%Here, we use the assumption that $\Loss(\vw)$ is scale invariant. Note that by scale invariance, $\rho_t \mSigma_{\vW_t} = \mSigma_{\hW_t}$. The derivation is deferred into appendix.
%\subsection{Effective Learning Rate}\label{subsec:effective_lr}

\iffalse 

\begin{lemma}
~\citep{li2020exp} shows that $\vw_{t+1} \gets \vw_t - \eta(1-\lambda_e)^{-2t} \left(\nabla \Loss(\vw_t) + \vxi_t \right)$
yields the same trajectory in function space as \Cref{eq:sgd-noisy}. In fact, they also correspond to the same surrogate SDE \Cref{eq:gamma_W,eq:gamma}, where the exponent in the rate schedule is the intrinsic LR. 
\end{lemma}
\fi 
%\begin{remark}[Connection to Exp LR]
%	SGD with Exp LR~\citep{li2020exp} yields the same surrogate SDE here, where the exponent in the rate schedule is the intrinsic LR. See derivation in Appendix.
%\end{remark}

%\begin{remark}[Connection to Adaptive Learning Rate Schedules]
%Note that \eqref{eq:gamma_W} and \eqref{eq:gamma-avg} can be viewed as spherical SDE with adaptive learning rate, which resembles RMSprop~\citep{hinton2012rmsprop}. The difference is that RMSprop adjusts LR coordinate-wise, while here it's adjusted globally.
%\end{remark}

Experimentally\footnote{\Cref{fig:7decay} shows that after a certain length of time the relationship $\gamma_t^{1/2} \propto \lambda_e^{-1/2}$ holds approximately, up to a small multiplicative constant. Since $\gamma_t$ is the running average of $\Tr(\Sigma_{\hW})$, the magnitude of the noise, it suggests for different regions of the landscape explored by SGD with different intrinsic LR $\lambda_e$, the noise scales don't differ a lot.} we find that the trace of noise is approximately constant. This is the assumption of the next lemma.  
%By contrast the assumption in the following lemma is much weaker, A special case is that the noise scale $\Tr(\Sigma_{\hW_t})$ is constant, i.e., $\Tr(\Sigma_{\hW}) = \sigma^2$ for all $\hW \in \sphS^{d-1}$. 
\begin{lemma}
If $\sigma^2 \le \Tr(\Sigma_{\hW}) \le (1+\eps)\sigma^2$ for all $\hW$ encountered in the trajectory, then
%$\gamma_t = \frac{\sigma^2}{2\lambda_e} + \left(\gamma_0 - \frac{\sigma^2}{2\lambda_e}\right) e^{-4\lambda_e t}$. 
\begin{equation}\label{eqn:norm_mixing2}
	\gamma_t = e^{-4 \lambda_et} \gamma_0 + \left(1 + O(\epsilon)\right) \frac{\sigma^2}{2\lambda_e}\left( 1 - e^{-4\lambda_e t}\right).
\end{equation}
Consequently
$\gamma_t^{1/2}$ converges to the stationary value $\frac{\sigma}{\sqrt{2 \lambda_e}}$ in $O(1/\lambda_e)$ time.
\end{lemma}
%In this case, we can solve for $\gamma_t$ by  suggesting that the effective LR 
	
%Unfortunately, $\Tr(\Sigma_{\hW_t})$ is not a constant in practice. Still, in 

%Our experiments lead to the following conjectures about the 
%In general, assuming $\gamma_t$ doesn't diverge (i.e. is bounded), integrating both sides of \Cref{eq:gamma} and dividing it by total time, we get $\frac{2}{T}\int_{t=0}^T \lambda_e\gamma_t \dd t = \frac{1}{T} \int_{t=0}^T \Tr(\Sigma_{\hW_t})\dd t$.


%  {\sc remove this conjecture?? Does it hurt anything else?}
%\begin{conjecture}[Conjecture from experiments, \Cref{fig:7decay}]
%	There is a small constant $\eps > 0$, such that with high probability $\sigma^2 \le \Tr(\Sigma_{\hW}) \le (1+\eps)\sigma^2$ for all $\hW$ that SDE visits.
%\end{conjecture}

% From~\eqref{eq:gamma-avg} we also get some insight into short term dynamics:

The lemma  again suggests that the initial effective LR decided together by learning rate $\eta$ and norm $\norm{\vW_0}$ only has a temporary effect on the dynamics: no matter how large is the initial effective LR, after $O(1/\lambda_e)$ time, the effective LR is always of the same magnitude $\Theta(\lambda_e^{1/2})$ ($\epsilon, \sigma$ are hidden as constants).
%\[
%	\frac{\sigma^2}{2 \lambda_e} \le \liminf_{t \to +\infty} \gamma_t \le \limsup_{t \to +\infty} \gamma_t \le \frac{C^2\sigma^2}{2 \lambda_e}
%\]
%\begin{equation}\label{eqn:norm_mixing2}
%	\left|\gamma_t - \frac{\sigma^2}{2\lambda_e}\right| \le  O(\eps) + \left(\gamma_0 - \frac{\sigma^2}{2\lambda_e}\right) e^{-4\lambda_e t}.
%\end{equation}

\begin{remark}[Intrisic LR and LR Decay] \label{rem:eff-int-lr}
    When decaying LR by $10$ in standard Step Decay schedules, the effective LR is temporarily reduced by a factor of $10$, but $\lambda_e^{-1/2}$ is only reduced by a factor of $\sqrt{10}$. Thus the effective LR will gradually increase by $\sqrt{10}$ times after the drop.
\end{remark}
\begin{remark}[Intrisic LR and the Final LR Decay] \label{rem:eff-int-lr-final}
    As observed in previous works (e.g., \citep{zagoruyko16wide,zhang2018three,li2020exp}, just to name a few), the train/test accuracy could first increase and then drop a little bit after LR decay, and the best test accuracy is usually achieved right after the final LR decay. \Cref{rem:eff-int-lr} can help to explain this by decomposing the training after the final LR decay into two stage. In the first stage, the effective LR is small, so the dynamics is more closer to the classical gradient flow approximation. In the second stage, the effective LR increases to the stationary value and brings larger noise and worse performance. This decomposition also works for earilier LR decay operations, but the phenomenon is more significant for the final LR decay because the intrinsic LR is much smaller.
\end{remark}

%\begin{remark}[The role of effective LR vs intrinsic LR] \label{rem:eff-int-lr}
%	For large intrinsic LR, the initial effective LR decided together by learning rate $\eta$ and norm $\norm{\vW_t}$ has only a temporary effect on the dynamics. For example, when decaying LR by $10$ in standard Step Decay schedules, the effective LR is divided by $10$, but its new stationary value is only roughly $\sqrt{10}$ times smaller since it is proportional to $\lambda_e^{-1/2}$. Thus the effective LR will eventually increase by $\sqrt{10}$ times after the drop. This explains the phenomenon that the train/test accuracy could first increase and then drop a little bit after LR decay as observed in previous works, e.g., \citep{zagoruyko16wide,zhang2018three,li2020exp} just to name a few.
%\end{remark}
%\begin{remark}
%	\Cref{rem:eff-int-lr} suggests we can participate the training after LR decay into two parts: the first part is transient and with much smaller noise, and thus is more closer to the classical gradient flow approximation, especially for the final LR decay, as the length of the first part is mainly determined by the magnitude of the intrinsic LR; the second part is stationary and with larger noise.
%\end{remark}



%\begin{remark}[Connection to AdamW] In Appendix, we will provide a theoretical analysis for AdamW, showing that  (Note in \Cref{eq:gamma}, $\gamma_0 = \frac{\norm{\vW_0}^4}{\eta^2}$. )
%\end{remark}


%With that said, the fluctuation of the effective learning rate $\gamma_t$ in each phase is even smaller than $\eps$, suggesting that 
%Let $r_t :=  (\lambda_e \gamma_t)^{-1/2} \sigma$. Then $r_t = \Theta(1)$ for $t \to +\infty$. The dynamics can be written as:
%\begin{equation}
%	\dd \hW_{t} = -\lambda_e^{1/2} \frac{r_t}{\sigma} \left(\nabla L\left(\hW_t\right)\dd t + \left(\mSigma_{\hW_t}\right)^{\frac{1}{2}} \dd B_t\right) - \frac{1}{2} \lambda_e r_t^2  \frac{\Tr(\Sigma_{\hW_t})}{\sigma^2} \hW_t\dd t.
%\end{equation}
%[explain here]

%\paragraph{Assumption 2:} The above dynamics of $\rho_t$ can be approximated by the following one:
%\begin{equation*}
%	\frac{\dd \gamma_t}{\dd t} = -4 \lambda_e \gamma_t + f(\gamma_t^{-0.5}), \label{eq:sde-rho_simplified}
%\end{equation*}
%
%where $f(\xi) = \E_{W\sim \mu_{\xi}} \left[ \Tr(\Sigma_{\hW_t}) \right]$, and $\mu_\xi$ is the stationary distribution of the following equation. 
%
%\begin{equation*}
%	\dd \hW_{t} = -\xi \left(\nabla L(\hW_t)\dd t + (\Sigma_{\hW_t})^{\frac{1}{2}} \dd B_t\right) - \frac{1}{2\xi^2}  \Tr(\Sigma_{\hW_t}) \hW_t\dd t.
%\end{equation*}

%Here, we assume $f(\xi)$ is monotone and upper bounded by some constant $C$.
% does not depend on $$, i.e., $\Sigma_{\hW_t} = \sigma^2 (I_d - \hW_t\hW_t^\top)$ for some $\sigma > 0$. Then $\Tr(\Sigma_{\hW_t}) = \sigma^2 (d-1)$.


%For further simplification, we will assume $\Sigma_{\hW_t} = I_d - \hW_t\hW_t^\top$. Thus $ \Tr(\Sigma_{\hW_t}) = d-1$. In this case, we can compute the stationary point of $\rho_t = \eta\sqrt{\frac{d-1}{2\lambda}}$. And thus we can see $\sqrt{\lambda}$ controls the LR of SGD on unit sphere after $\rho_t$ converges. 

%\subsection{The Fast equilibrium conjecture: Converging in $O(1/\eta\lambda)$ steps}


%This dynamics already 
\subsection{A conjecture about mixing time in function space}\label{subsec:conjecture}
As mentioned earlier, SGD may take a very long time to mix in the parameter space. However, we observed that test/train accuracy and loss converge in expectation soon after the norm $\norm{\vW_t}$ converges in expectation, which only takes $O(1/\lambda_e)$ time through our theoretical analysis.

%within a much shorter time.
%In fact, our experiments suggest the convergence for the test/train accuracies and losses occurs soon after the norm $\norm{\vW_t}$ converges in expectation.

%the convergence of  is much faster in practice
%\citep{shi2020learning}
%make  the training loss converge in expectation. Intriguingly, we found that the convergence speed is much faster in practice. In fact, our experiments suggest the convergence for the test/train accuracies and losses occurs soon after the norm $\norm{\vW_t}$ converges in expectation. %Here the convergence means convergence in distribution: due to the noise, we should not expect the accuracy and loss converge to some constant like the norm, but it turns out they seem to follow the same distribution. (over the randomness of batches and (init???)) 

%An intriguing experimental observation is that as the effective learning rate $\gamma_t^{-0.5}$, or equivalently the norm $\rho_t^{0.5}$ converges to some constant,  the test/train accuracies and losses also seem to converge to some equilibrium distribution, which is much faster than the existing convergence analysis \citep{shi2020learning}, where the mixing time is exponential to $\frac{1}{\eta}$.

More specifically, we find experimentally that the number of steps of SGD (or the length of time for SDE) after the norm converges doesn't affect the expectation of any known statistics related to the training procedure, including train/test accuracy and loss, and it doesn't affect the output distribution on any single data. This means the neural net reaches an ``equilibrium state'' after a number of SGD steps, which also matches with the common impression that SGD will oscillate at some plateau at the end of each phase in Step Decay schedule, and that staying longer at the plateau does not harm the generalization.

The above findings motivate us to define the notion of ``equilibrium state'' rigorously and make a conjecture formally. %For the above variant of \eqref{eq:SDE_wd} allowing time-varying LR and WD, 
For a random variable $X$, we define $P_{X}$ to be the probability distribution of $X$. The total variation $\dTV(P_1, P_2)$ between two probability measures $P_1, P_2$ is defined by the supremum of $\lvert P_1(A) - P_2(A) \rvert$ over all measurable set $A$. Given input $\vx$ and neural net parameter $\vw$, we use $F(\vw; \vx)$ to denote the output of the neural net (which is the pre-softmax logits in classification tasks).
%Our conjecture is formally stated below:
%describing the evolution of the distribution of $\vW_t$ in the following way: $\vW_t \sim T_{\vlambda_{\bm{e}},\veta}(t; \mu)$, where $\vW_0\sim \mu$. Specifically, we use $T_{\vlambda_{\bm{e}},\veta}$ to denote the operator with constant $\lambda_e,\eta$.
%In detail, for the above variant of \eqref{eq:SDE_wd} allowing time-varying LR and WD, we define the operator $T_{\vlambda_{\bm{e}},\veta}$ describing the evolution of the distribution of $\vW_t$ in the following way: $\vW_t \sim T_{\vlambda_{\bm{e}},\veta}(t; \mu)$, where $\vW_0\sim \mu$. Specifically, we use $T_{\vlambda_{\bm{e}},\veta}$ to denote the operator with constant $\lambda_e,\eta$.
\begin{conjecture}[The Fast Equilibrium Conjecture] \label{conj:weaker}
	%Under the dynamics of \eqref{eq:gamma_W} and \eqref{eq:SDE_wd}, modern neural nets converges to the equilibrium distribution in function space in $O(1/\lambda_e)$ time. In other words, for $t\ge \Omega(1/\lambda_e)$, any $t'\ge 0$, any $\mu_1,\mu_2$, any $\lambda_e(t),\eta(t)$, any data $(\vx, y)$ and loss function $\ell(\cdot, \cdot)$, we have
	Under the dynamics of \eqref{eq:gamma_W} and \eqref{eq:gamma}, modern neural nets converge to the equilibrium distribution in $O(1/\lambda_e)$ time in the following sense. Given two initial distributions $\mu, \mu'$ for $\vW_0$, constant learning rate and effective weight decay schedules $\lambda_e^*, \eta^*$, there exists a mixing time $T = O(1 / \lambda^*_e)$ such that for any input data $\vx$ from some input domain $\mathcal{X}$,
	\[
		\forall t \ge T: \qquad \dTV\left(P_{F\left(\vW_t;~\vx\right)}, P_{F\left(\vW'_t;~\vx\right)} \right) \approx 0,
	\]
	where $\vW_t \sim \nu(\mu; \lambda_e^*, \eta^*, t)$, $\vW'_t \sim \nu(\mu'; \lambda_e^*, \eta^*, t)$.
	%in function space in $O(1/\lambda_e)$ time. In other words, for $t\ge \Omega(1/\lambda_e)$, any $t'\ge 0$, any $\mu_1,\mu_2$, any $\lambda_e(t),\eta(t)$, any data $(\vx, y)$ and loss function $\ell(\cdot, \cdot)$, we have
	%\begin{equation}
	%\E_{\nu_1}\left[ \ell(f(\vW; \vx), y)\right]	 \approx \E_{\nu_2}\left[ \ell(f(\vW; \vx), y)\right],
	%\end{equation}
	%where $\nu_i = T'_{\vlambda_{\bm{e}},\veta}(t'; T(t;\mu_i))$, $i=1,2$ and $f(\vW,\vx)$ is the output of the neural net on input $\vx$ with weight $\vW$.
\end{conjecture}

%\begin{remark}
	It is worth to note that this conjecture obviously does not hold for some pathological initial distributions, e.g., all the neurons are initially dead. But we can verify that our conjecture holds for many initial distributions that can occur in training neural nets, e.g., random initialization, or the distribution after training with certain schedule for certain number of epochs. It remains a future work to theoretically identify the specific condition for this conjecture.
%\end{remark}


\subsection{What happens in real life training -- An interpretation} \label{sec:twop}
%\subsection{Approximating the Last LR Decay by Gradient Flow}

%In practice, we find that the Step Decay schedule reaches the equilibrium in each phase, and that the best test accuracy is achieved right after the final LR decay, which is a common feature (or it could be a continuous but quick drop) for SOTA LR schedules, including Cosine~\citep{loshchilov2016sgdr} and 1-cycle cyclic LR~\citep{smith2019super}. 
%The reason is that the small intrinsic LR  makes the stochastic process take very long time to decrease the norm of the weights. And before the norm converges to the new stationary value, the tiny effective LR significantly reduced the noise so full training accuracy is quickly reached. This fits with the traditional view of approximating SGD with small LR by Gradient Flow.


Let's first recap the Step Decay schedule --  LR in each phase is $\bar{\eta_i}$ where there are total $K$ phases. In this subsection, we will further extend our discussion to general LR and WD schedules, i.e. for learning rate schedule $\eta(t)$ and effective weight decay schedule $\lambda_e(t)$, we define $\nu(\mu; \lambda_{e},\eta, t)$ to be the marginal distribution of $\vW_t$ in the following SDE when $\vW_0 \sim \mu$:
%Based on our observation from the experiments, 
%We further find that the output distribution on any single data, or even the improvement of the test accuracy under further training with a possibly time-varying LR schedule or WD schedule.
\begin{equation} \label{eq:SDE_wd}
\dd \vW_{t} = - \eta(t) \left(\nabla \Loss(\vW_t)\dd t + (\mSigma_{\vW_t})^{\frac{1}{2}} \dd \vB_t\right) - \lambda_e(t) \vW_t\dd t.
\end{equation}

Interesting, we empirically find that the above conjecture still holds even if we are allowed to fine-tune the model before producing the output. This can be modeled by starting another SDE from $t \ge T$ with a different pair of LR and effective WD schedules $\tilde{\eta}(\tau), \tilde{\lambda}_e(\tau)$:
%, or even the improvement of the test accuracy under further training with a possibly time-varying LR schedule or WD schedule
%Indeed, empirically we observe an even strong form of equilibrium:
\begin{conjecture}[The Fast Equilibrium Conjecture, Strong Form]
	Let  $\tilde{\eta}(\tau), \tilde{\lambda}_e(\tau)$ be a pair of learning rate and effective weight decay schedules. Under the same conditions of \Cref{conj:weaker}, there exists a mixing time $T = O(1 / \lambda^*_e)$ such that for any input data $\vx$ from some input domain $\mathcal{X}$,
	\[
		\forall t \ge T: \qquad \dTV\left(P_{F\left(\vW_{t, \tau};~\vx\right)}, P_{F\left(\vW_{t, \tau}';~\vx\right)} \right) \approx 0,
	\]
	where $\vW_{t,\tau} \sim \nu\left(\nu(\mu; \lambda_e^*, \eta^*, t); \tilde{\lambda}_e, \tilde{\eta}, t\right)$, $\vW'_{t, \tau} \sim \nu\left(\nu(\mu'; \lambda_e^*, \eta^*, t); \tilde{\lambda}_e, \tilde{\eta}, t\right)$.
\end{conjecture}

%\kaifeng{I split the fast equilibrium conjecture into a weaker form and a stronger form. I think it makes the conjecture easy to read and understand}

%\begin{remark}
	In Appendix we provide the discrete version of the  conjecture by viewing each step of SGD as one step transition of a Markov Chain. By this mean the conjecture can be extended  to momentum SGD. 	
%\end{remark}


Hence, the above conjecture suggests the generalization error of Step Decay schedule only depends on the intrinsic LR for its last equilibrium. As the training time in every phase is quite long (e.g., in \citep{he2016deep,zagoruyko16wide} SGD enters the next phase when the error plateaus) except that early stopping after the final LR decay is essential for achieving the best performance (as discussed in ~\Cref{rem:eff-int-lr-final}), the last equilibrium is most likely achieved in the second last phase. Thus, Step Decay could be abstracted into the following general \emph{two-phase training} paradigm, where the only hyper-parameter of SGD that affects generalization is the intrinsic LR, $\lambda_e$:
\begin{enumerate}
\item \textbf{SDE Phase.} Reach the equilibrium of (momentum) SGD with $\lambda_e$ (as fast as possible).
\item \textbf{Gradient Flow Phase.} Decay the learning rate by a large constant, e.g., 10, and set $\lambda_e=0$. Train until loss is zero. %at full training accuracy.
\end{enumerate}
The above training paradigm  says for good generalization, what we need is only \emph{reaching the equilibrium of small (intrinsic) LR and decaying LR}. As a sanity check, we show that the initial large LR is not necessary to achieve high test accuracy, i.e., networks trained directly with the small intrinsic LR, with a longer training budget, could also achieve the same performance. See \Cref{fig:small_lr_sota}.
 
%\paragraph{So what's the benefit of early large learning rates?} 
\textbf{So what's the benefit of early large learning rates?} In Appendix we show that the the large (intrinsic) LR in early phase allows the network to get rid of the affect of potentially unfavorable initialization quickly and thus gets much consistent and robust behavior for different initialization method. This matches the common impression that the training of modern deep nets is not sensitive to initialization. From this point of view, Step Decay with large initial LR is a good heuristic to achieve the desired equilibrium quickly. Also see \Cref{fig:small_lr_sota} for that initial large (intrinsic) LR helps the red line to reach the equilibrium of $\lambda_e = 0.1\times 0.0005$ much faster than other settings without large intrinsic LR in early phases.

%\paragraph{But is it worth waiting for the equilibrium of small (intrinsic) LR?} 



\textbf{But is it worth waiting for the equilibrium of small (intrinsic) LR?} In \Cref{fig:which_equilibrium} we show that different equilibrium does lead to different performance after the final LR decay. Given this experimental result we speculate the basins of different scales in the optimization landscape seems to be nested, i.e. a larger basin can contain multiple smaller basins of different performances. And reaching the equilibrium of a smaller intrinsic LR seems to be a stronger regularization method, though it also costs much more time.


\textbf{Connection to AdamW:} \citep{loshchilov2018decoupled} found that using the parametrization of $\lambda_e = \eta\lambda$  achieves better generalization and a more separable hyper-parameter search space for SGD and Adam, which are named SGDW and AdamW. So far we've justified the role of intrinsic LR and that initial LR is of limited importance for SGD(W). The theorem below shows that the notion of intrinsic LR also makes sense for AdamW.
\begin{theorem}
For scale-invariant loss $\Loss$, multiplying the initial weight $\vW_0$ and the learning rate by the same constant would not change the trajectory of AdamW in function space.
\end{theorem}

% \begin{figure}
%         \centering
% 		\includegraphics[width=0.6\textwidth]{tmp_images/which_equilibrium}
%         \caption{\small Equilibrium of smaller intrinsic LR leads to higher test accuracy on CIFAR after LR decay by 10. PreResNet32 trained with SGD without momentum and with WD factor 0.0005.}
%         \label{fig:which_equilibrium}
% \end{figure}


\begin{figure}
        \centering
        \begin{subfigure}[b]{0.23\textwidth}
                \centering
				\includegraphics[width=\linewidth]{tmp_images/small_lr_train}
				\caption{Train accuracy}
        \end{subfigure}%
        \begin{subfigure}[b]{0.23\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/small_lr_test}
                \caption{Test accuracy}
        \end{subfigure}%
        \begin{subfigure}[b]{0.23\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/small_lr_norm}
                \caption{Norm}
        \end{subfigure}%
        \begin{subfigure}[b]{0.30\textwidth}
                \centering
                \includegraphics[width=\linewidth]{tmp_images/which_equilibrium.png}
                \caption{Train/Test Accuracy}
                \label{fig:which_equilibrium}
        \end{subfigure}%
        \caption{\small(a)-(c)  Achieving SOTA test accuracy by $0.9$-momentum SGD with small learning rates (the blue line). The initial learning rate is 0.1, initial WD factor is 0.0005. The label \texttt{wd\_x\_y\_lr\_z\_u} means dividing WD factor by 10 at epoch $x$ and $y$, and dividing LR by 10 at epoch $z$ and $u$. For example, the blue line means dividing LR by 10 twice at epoch 0, i.e. using an initial LR of 0.001 and dividing LR by 10 at epoch 5000. The red line is baseline. (d). Equilibrium of smaller intrinsic LR leads to higher test accuracy on CIFAR after LR decay by 10. PreResNet32 trained with SGD without momentum and with WD factor 0.0005. }
        \label{fig:small_lr_sota}
\end{figure}
%The popular learning rate schedules achieving SOTA performances, such as Step Decay, Cosine~\citep{loshchilov2016sgdr}, and 1-cycle cyclic LR~\citep{smith2019super} share a common feature -- arrive (after many epochs) at a small LR, then switch to a tiny LR, train for  a short period of time and stop. Training accuracy is seen to go to $100\%$ and the test accuracy also peaks. 
%
%\emph{How does the final phase with tiny LR fit into our SDE framework?}
%The short answer is, SGD in the final phase with tiny LR should be approximated as Gradient Flow, rather than SDE. The reason is that with such a small intrinsic LR led by small LR, the stochastic process takes very long time to decrease the norm of the weights. And before the norm converges to the new stationary value, the tiny effective LR significantly reduced the noise so the dynamics reaches the training accuracy quickly. This fits with the traditional view of approximating SGD with small LR by Gradient Flow. A more detailed discussion could be found in 
%	\Cref{sec:two-phases}.
	

==> two_phase.tex <==
\section{A New Training Paradigm with Two Phases} \label{sec:two-phases}

	In \Cref{sec:theory} and \Cref{sec:evidence}, we've shown both theoretical and experimental evidence that the equilibrium determined by the intrinsic learning rate is independent of training history and controls the future performance of the network, e.g. the improvement of test accuracy after another LR decay. Thus it's natural to propose  the following conceptually simpler \emph{two-phase training paradigm}, where Step Decay LR schedule can be viewed as a realization of the new paradigm.
	
\paragraph{A Two-Phase Training Paradigm:}Pick a suitable intrinsic learning rate $\lambda_e=\eta\lambda$.
\begin{enumerate}
\item \textbf{SDE Phase.} Reach the equilibrium of (momentum) SGD with $\lambda_e$, as fast as possible.
\item \textbf{Gradient Flow Phase.} Decay the learning rate by a large constant, e.g. 10, and set $\lambda_e=0$. Train until loss is zero. %at full training accuracy.
\end{enumerate}

Philosophically, one can think the goal of the first phase is to pick a good initialization for the second by leveraging the regularization effect from the noise in SDE. Good initialization can be those networks in wider minima, or can have some other unknown benefits which ensures better generalization in its neighborhood. And then we fine tune the network in the second phase. [This view is slightly different from existing works???]
	Note that setting $\lambda_e=0$ (or the classic weight decay $\eta=0$) is usually optional in practice, and indeed it could be replaced by a continuous but quick drop in LR \citep{smith2019super}.
	
	%The reason behind this is that with a smaller effective LR the network can achieve full training accuracy quickly, before the regularization effect of the decreased effective weight decay occurs. [Need a simple calculation ??

\paragraph{The benefit of early large learning rates.} In Appendix we show that the the large (intrinsic) LR in early phase allows the network to get rid of the affect of potentially unfavorable initialization quickly and thus gets much consistent and robust behavior for different initialization method. This matches the common impression that the training of modern deep nets is not sensitive to initialization. From this point of view, Step Decay with large initial LR is a good heuristic to achieve the desired equilibrium quickly. Also see \Cref{fig:small_lr_sota} for that initial large (intrinsic) LR helps the red line to reach the equilibrium of $\lambda_e = 0.1\times 0.0005$ much faster than other settings without large intrinsic LR in early phases.








==> unorganized.tex <==

\begin{comment}
\section{Useful disorganized points}

\subsection{Connection to adaptive LR}

Large learning rate is sort of regularization, 

Normalized BN-SGD + RMS-Prop[cite, hinton's notes] (which is ADAM \citep{kingma2014adam} with $\beta_1 = 0$) = BN-SGD

connection to \citep{loshchilov2018decoupled}. (related work)

discussion: what's the potential effect of double RMS-prop?? (Minor, appendix)

AdamW: $\rho_t^{0.5} \sim \lambda^{-0.5}*\alpha$, $\dd W /\dd t\sim \alpha$, thus the intrinsic lr is also $\dd \hat{W}_t /\dd t\sim \lambda^{0.5}$. 



\section{Disorganized}
	
	\zhiyuan{ Maybe the two phases of the new dynamics can be understood as GF and SDE respectively. Each time we decays $\eta$, we enter the GF phase. When it converges, it goes back to SDE phase. The time for convergence might be $O(1/\lambda)$.}
	
	\[L(w) = \E_{\xi\sim N(0,I_d)}[\xi^\top w]=0.\]
	
	\[ L'(w_1,w_2) = L(\frac{w_1}{|w_1|}+\frac{w_2}{|w_2|}).\]
	
	
	%   Two dynamics:
	%   \begin{itemize}
	%       \item shared noise: converge to the same vector
	%       \item independent gaussian noise: independent trajectories
	%   \end{itemize}
	
	
	
	
	
	Exp LR continuous: The equivalence built between SGD + ExpLR and SGD + WD + BN can be extended to the continuous case. By the same approximation, we have 
	
	\begin{itemize}
		\item  ExpLR SGD: $W_{t+1} = W_t - \eta_t \left(\nabla L(W_t) + \xi_t\right)$, where $\xi_t \sim N(\bm{0}, \Sigma_{W_t})$.
		
		\item ExpLR SDE: $\dd W_{t} = - \eta_t \left(\nabla L(W_t) \dd t+ (\Sigma_{W_t})^{\frac{1}{2}} \dd B_t\right)$.
	\end{itemize}
	
	
	Define $\hW_t = \frac{W_t}{\norm{W_t}_F}$, $\rho_t = \norm{W_t}_F^2$, and by Ito's Lemma, we have 
	
	\[\dd \hW_{t} = - \frac{\eta_t}{\rho_t} \left(\nabla L(\hW_t)\dd t + (\Sigma_{\hW_t})^{\frac{1}{2}} \dd B_t\right) - \frac{\eta_t^2}{2\rho_t^2}  \Tr{\Sigma_{\hW_t}} \hW_t\dd t.\] 
	
	\[\frac{\dd \rho_t}{\dd t} = -2\lambda \rho_t + \frac{\eta_t^2}{\rho_t}\Tr{\Sigma_{\hW_t}}.\]
	
	Smooth approximation: 
	
	SGD == SDE: 
	
	
	SDE approximation of GD: 
	
	\begin{itemize}
		\item GD:	$W_{t+1} = W_t - \eta \nabla L(W_t)$.
		\item SDE:	$\dd W_{t} = - \eta \left(\nabla L(W_t)\dd t + \nabla L(W_t) \dd B_t\right)$.
	\end{itemize}

	For quadratic loss $L(W) = \frac{1}{2} W^\top A W$,  \[L(W_{t+1}) - L(W_t) = -\eta \norm{\nabla L(W_t)}^2_2 + \frac{\eta^2}{2} \nabla L(W_t)^\top (\nabla^2 L(W_t)) \nabla L(W_t).\] \[\E[d L(W_t)] =\E[(-\eta \norm{\nabla L(W_t)}_2^2 + \frac{\eta^2}{2} \nabla L(W_t)^\top (\nabla^2 L(W_t)) \nabla L(W_t)) \dd t].\]
	%\section{Relationship with Stochastic Weight Averaging }
	
\end{comment}


The concept of the equilibrium can be understood in another way: given two networks from two possibly different initial distribution, if we train them with SGD with the same $\lambda_e$ for enough long time, then there's no statistics which only uses the current network or future network (possibly trained by SGD with a different schedule) as a black-box to distinguish them. 

However, the conjecture is not saying that even if we open the black-box, we still cannot distinguish them.
